Lutz's Spoiler Technique Revisited: A Unified Approach to Worst-Case Optimal Entailment of Unions of Conjunctive Queries in Locally-Forward Description Logics

We present a unified approach to (both finite and unrestricted) worst-case optimal entailment of (unions of) conjunctive queries (U)CQs in the wide class of "locally-forward" description logics. The main technique that we employ is a generalisation of Lutz's spoiler technique, originally developed for CQ entailment in ALCHQ. Our result closes numerous gaps present in the literature, most notably implying ExpTime-completeness of (U)CQ-querying for any superlogic of ALC contained in ALCHbregQ, and, as we believe, is abstract enough to be employed as a black-box in many new scenarios.

==> graphics/metaproperties-figure-forward-unrav-example-LHS.tex <==
%!TEX root = ../../main.tex

\begin{tikzpicture}[transform shape]
    \draw (0,1) node[ptrond, jaune, label=center:\small{1}] (A1) {\phantom{0}};

    \draw (1.4, 2) node[ptrond, vert, label=center:\small{2}] (A2) {\phantom{0}};
    \node[] at (1.4, 2.5) {\(\indva \)};

    \draw (2.4, 0.6) node[ptrond, vert, label=center:\small{3}] (A3) {\phantom{0}};
    \node[] at (2.4, 0.0) {\(\indvc \)};

    \draw (3.2, 1.6) node[ptrond, rouge, label=center:\small{4}] (A4) {\phantom{0}};
    \node[] at (3.7, 1.6) {\(\indvb \)};

    \path[->] (A1) edge [loop left, red] node[xshift=2] {\small\(\roler \)} (A1);
    \path[->>,dashdotdotted] (A1) edge [bend left=30, blue] node[yshift=4] {\small\(\roles \)} (A2);

    \path[->] (A2) edge [red] node[yshift=-3, xshift=2] {\small\(\roler \)} (A1);
    \path[->] (A2) edge [bend left=30, red] node[yshift=4] {\small\(\roler \)} (A4);

    \path[->] (A3) edge [red] node[yshift=4.5,xshift=2] {\small\(\roler \)} (A2);
    \path[->] (A3) edge [bend left=10, red] node[yshift=3] {\small\(\roler \)} (A1);
    \path[->] (A3) edge [bend right=30, red] node[xshift=4] {\small\(\roler \)} (A4);

    \path[->>,dashdotdotted] (A4) edge [loop above, blue] node {\small\(\roles \)} (A4);
    \path[->>,dashdotdotted] (A4) edge [bend right=30, blue] node[xshift=-2.5,yshift=1.5] {\small\(\roles \)} (A3);

    \node[] at (0, -0.6) {\(\phantom{0} \)};

\end{tikzpicture}

==> graphics/metaproperties-figure-forward-unrav-example-RHS.tex <==
%!TEX root = ../../main.tex

\begin{tikzpicture}[scale=0.6, transform shape]
      \draw (0,-2) node[ptrond, vert, label=center:\small{12}] (A12) {\phantom{0000}};
      \draw (-2,-4) node[ptrond, jaune, label=center:\small{121}] (A121) {\phantom{0000}};
      \draw (0,-4) node[ptrond, rouge, label=center:\small{124}] (A124) {\phantom{0000}};
      \draw (-2, -6) node[ptrond, vert, label=center:\small{1212}] (A1212) {\phantom{0000}};
      \node[] at (-2, -6.75) {\(\ldots \)};
      \draw (0, -6) node[ptrond, vert, label=center:\small{1243}] (A1243) {\phantom{0000}};
      \node[] at (0, -6.75) {\(\ldots \)};

      \path[->] (A12) edge [red] node[xshift=-6] {\(\roler \)} (A121);
      \path[->] (A12) edge [red] node[xshift=6] {\(\roler \)} (A124);
      \path[->] (A121) edge [loop left, red] node[xshift=-3] {\(\roler \)} (A121);
      \path[->>,dashdotdotted] (A124) edge [loop right, blue] node[xshift=4] {\(\roles \)} (A124);
      \path[->>,dashdotdotted] (A121) edge [blue] node[xshift=-4] {\(\roles \)} (A1212);
      \path[->>,dashdotdotted] (A124) edge [blue] node[xshift=4] {\(\roles \)} (A1243);

      \draw (4, 0) node[ptrond, vert, label=center:\small{2}] (A2) {\phantom{0000}};
      \node[] at (3.25, 0) {\(\indva \)};

      \draw (4, -2) node[ptrond, jaune, label=center:\small{21}] (A21) {\phantom{0000}};
      \draw (4, -4) node[ptrond, vert, label=center:\small{212}] (A212) {\phantom{0000}};
      \draw (3, -6) node[ptrond, jaune, label=center:\small{2121}] (A2121) {\phantom{0000}};
      \node[] at (3, -6.75) {\(\ldots \)};
      \draw (5, -6) node[ptrond, rouge, label=center:\small{2124}] (A2124) {\phantom{0000}};
      \node[] at (5, -6.75) {\(\ldots \)};

      \path[->] (A2) edge [red] node[xshift=-5] {\(\roler \)} (A21);
      \path[->] (A21) edge [loop right, red] node[xshift=-2] {\(\roler \)} (A21);
      \path[->>,dashdotdotted] (A21) edge [blue] node[xshift=4] {\(\roles \)} (A212);
      \path[->] (A212) edge [red] node[xshift=-4] {\(\roler \)} (A2121);
      \path[->] (A212) edge [red] node[xshift=4] {\(\roler \)} (A2124);
      \path[->] (A2121) edge [loop left, red] node[xshift=-1] {\(\roler \)} (A2121);
      \path[->>,dashdotdotted] (A2124) edge [loop right, blue] node[xshift=1] {\(\roles \)} (A2124);

      \draw (9.25, 0) node[ptrond, vert, label=center:\small{3}] (A3) {\phantom{0000}};
      \node[] at (10, 0) {\(\indvc \)};

      \draw (9.25, -2) node[ptrond, jaune, label=center:\small{31}] (A31) {\phantom{0000}};
      \draw (9.25, -4) node[ptrond, vert, label=center:\small{312}] (A312) {\phantom{0000}};
      \draw (8.25, -6) node[ptrond, jaune, label=center:\small{3121}] (A3121) {\phantom{0000}};
      \node[] at (8.25, -6.75) {\(\ldots \)};
      \draw (10.25, -6) node[ptrond, rouge, label=center:\small{3124}] (A3124) {\phantom{0000}};
      \node[] at (10.25, -6.75) {\(\ldots \)};

      \node[] at (2, -2) {\(\ldots \)};

      \path[->] (A3) edge [red] node[xshift=-5] {\(\roler \)} (A31);
      \path[->] (A31) edge [loop right, red] node[xshift=2] {\(\roler \)} (A31);
      \path[->>,dashdotdotted] (A31) edge [blue] node[xshift=4] {\(\roles \)} (A312);
      \path[->] (A312) edge [red] node[xshift=-4] {\(\roler \)} (A3121);
      \path[->] (A312) edge [red] node[xshift=4] {\(\roler \)} (A3124);
      \path[->] (A3121) edge [loop left, red] node {\(\roler \)} (A3121);
      \path[->>,dashdotdotted] (A3124) edge [loop right, blue] node[xshift=1] {\(\roles \)} (A3124);

      \draw (6.5, 1) node[ptrond, rouge, label=center:\small{4}] (A4) {\phantom{0000}};
      \node[] at (6.5, 1.75) {\(\indvb \)};


      % Abox roles
      \path[->>,dashdotdotted] (A4) edge [loop below, blue] node[xshift=-15, yshift=9] {\(\roles \)} (A4);
      \path[->] (A2) edge [bend left=30, red] node[yshift=4] {\small\(\roler \)} (A4);
      \path[->] (A3) edge [bend left=30, red] node[yshift=4.5,xshift=2] {\small\(\roler \)} (A2);
      \path[->] (A3) edge [bend right=30, red] node[xshift=4, yshift=4] {\small\(\roler \)} (A4);
      \path[->>,dashdotdotted] (A4) edge [bend right=30, blue] node[xshift=4,yshift=4] {\small\(\roles \)} (A3);
\end{tikzpicture}

==> sections/applications.tex <==
%!TEX root = ../main.tex

\section{Applications}\label{sec:applications}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Forward unravellings and forward DLs}\label{subsec:forward-unrav-and-forward-dls}

Forward unravellings make interpretations forest-shaped while preserving their named components.
Such a notion differs only slightly from the classical unravellings (consult~\cite[Def. 3.21]{dlbook}). 
The crucial difference is that their preserve selected naming components, \ie{} that the sequences starting from two named individuals are excluded from the domain and that the roles linking named individuals are assigned manually by the last item from \cref{def:omega-fwd-unrav}. 
Before reading the definition we suggest consulting \cref{fig:forward-unrav-example}. 

\begin{definition}\label{def:omega-fwd-unrav} 
  Let \(\names \subseteq \Ilang \) be a non-empty set of individual names.
  An $\names$-rooted \newnotion{forward unravelling} of an interpretation~\(\interI \) is an interpretation 
  \(\interomegafwdunravInames = (\DeltaomegafwdunravInames, \cdotomegafwdunravInames) \) satisfying all the following conditions:
  \begin{enumerate} \itemsep0em 
    \item\label{item:domain:def:omega-fwd-unrav} Its domain consists of all non-empty words of elements from \(\DeltaI \) starting from \(\names \)-named elements, except those, where the first two elements are \(\names \)-named.
    In symbols: 
    \[
    \DeltaomegafwdunravInames = \DeltaInamednames \cdot {(\DeltaI)}^{*} \; \setminus \; \Big(~\DeltaInamednames \cdot \DeltaInamednames \cdot {(\DeltaI)}^{*} \; \Big).
    \]
    For convenience, we do not syntactically distinguish elements from \(\DeltaI \) and single-letter words from \(\DeltaomegafwdunravInames \). 
    In particular, it means that \(\DeltaInamednames \subseteq \DeltaomegafwdunravInames \). 
    The last element of \(\wordw \in \DeltaomegafwdunravInames \) is denoted with \(\lastw \).
  %
    \item\label{item:names:def:omega-fwd-unrav} For all individual names \(\indva \in \names \) we have \({\indva}^{\interomegafwdunravInames} = {\indva}^{\interI} \) and for all other names \(\indva \in \Ilang \setminus \names \) there exists an individual name \(\indvb \in \names \) satisfying \(\indva^{\interomegafwdunravInames} = \indvb^{\interomegafwdunravInames} \).
  %
    \item\label{item:concepts:def:omega-fwd-unrav} For any concept name \(\conceptA \in \Clang \) the equality \({\conceptA}^{\interomegafwdunravInames} = \set{\wordw \mid \lastw \in {\conceptA}^{\interI}} \) holds.
  % %
    \item\label{item:roles:def:omega-fwd-unrav} For all role names \(\roler \in \Rlang \) we define \({\roler}^{\interomegafwdunravInames} \) as the intersection of \(\DeltaomegafwdunravInames \times \DeltaomegafwdunravInames \) and the set
    \[
    \Big( {\roler}^{\interI} \cap (\DeltaInamednames \times \DeltaInamednames) \Big) \cup 
    \Big \{ (\wordw,\wordw \cdot \domelemd) \mid (\lastw, \domelemd) \in {\roler}^{\interI} \Big \}. \label{eq:roles-omega-fwd-unrav} \tag{\mbox{\(\dagger \)}}
    \] 
    Intuitively, the above set is composed of two parts, where the first component preserves all possible connections between \(\names \)-named elements and the second one preserves roles, mimicking the classical unravelling. 
  \end{enumerate}
\end{definition}
%
\begin{figure}[ht]
  \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \input{graphics/metaproperties-figure-forward-unrav-example-LHS}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.6\textwidth}
    \input{graphics/metaproperties-figure-forward-unrav-example-RHS}
  \end{subfigure}
  \caption{An interpretation \(\interI \) (LHS) with a fragment of its \(\set{\indva, \indvb, \indvc} \)-rooted forward unravelling \(\interomegafwdunravI{\set{\indva, \indvb, \indvc}} \) (RHS). Two nodes in the picture have the same colour if and only if they satisfy the same atomic concepts. [TODO CHANGE PICTURES]}\label{fig:forward-unrav-example}
\end{figure}

Forward unravellings clearly produce forest-shaped interpretations, in the following sense:
%
\begin{lemma}\label{lemma:fwd-unrav-are-forests}
The \(\names \)-rooted forward unravellings \(\interomegafwdunravInames \) of \(\interI \) are \(\names \)-rooted forward forests.
\end{lemma}
%
\begin{proof}
More precisely, \(\interomegafwdunravInames \) is an \(\names \)-rooted \(\DeltaI \)-forest.
To see that \(\interomegafwdunravInames \) is a forest we observe that its domain is prefix-closed (follows from \cref{item:domain:def:omega-fwd-unrav} of \cref{def:omega-fwd-unrav}) and that it satisfies all forests' criteria on roles (by \cref{item:roles:def:omega-fwd-unrav} of \cref{def:omega-fwd-unrav}).
The \(\names \)-rootedness follows from \cref{item:names:def:omega-fwd-unrav} \cref{def:omega-fwd-unrav}.
\end{proof}

